Dimension Independent and Computationally Efficient Shadow Tomography

We describe a new shadow tomography algorithm that uses $n=\Theta(\sqrt{m}\log m/\epsilon^2)$ samples, for $m$ measurements and additive error $\epsilon$, which is independent of the dimension of the quantum state being learned. This stands in contrast to all previously known algorithms that improve upon the naive approach. The sample complexity also has optimal dependence on $\epsilon$. Additionally, this algorithm is efficient in various aspects, including quantum memory usage (possibly even $O(1)$), gate complexity, classical computation, and robustness to qubit measurement noise. It can also be implemented as a read-once quantum circuit with low quantum memory usage, i.e., it will hold only one copy of $\rho$ in memory, and discard it before asking for a new one, with the additional memory needed being $O(m\log n)$. Our approach builds on the idea of using noisy measurements, but instead of focusing on gentleness in trace distance, we focus on the \textit{gentleness in shadows}, i.e., we show that the noisy measurements do not significantly perturb the expected values.

==> para_other_props.tex <==
\paragraph{Other properties:} Note that our analysis considers the worst case. So, for many choices of the POVM's $M_1\dots M_m$, the inequalities will not be tight, which means that in certain cases, our techniques might lead to a smaller sample complexity for our algorithm. Consider the case when all the commutators have their norm bounded by some $C_{max}$. Then, if we use Lemma \ref{lem_conjugate_bound} instead of $\ref{lem_exp_first_order}$ to bound the deviations in Section \ref{sec_bnd_dv}, we get that up to a change in the defined universal constants, we can upper bound the expression in Equation \ref{eqn_first_order_prob} by 
\[2\exp\left(-\frac{\epsilon^2n^2}{2mkc_1^2C_{max}^2}\right),\] and upper bound $S_{2,j}$ in Section \ref{sec_bnd_dv} by $c_2\frac {\lambda^2}{n^2}C_{max}$. This means that the constraints in Theorem \ref{thm_sample_cmpl} are replaced by:
\begin{itemize}
        \item $k=c_0\frac 1 {\epsilon ^2}\log\frac 1{\delta}$.
        \item $n\geq 10k$.
        \item $n^2\geq 8c_1^2C_{max}^2mk\frac 1 {\epsilon^2}\log \frac 1 \delta  $.
        \item $c_2C^2\frac{mk}{n^2}C_{max}\ln 2+c_2C^2C_{max}\frac k {n^2}\ln \frac 1 \delta\leq \epsilon $,
\end{itemize}

 which implies that the sample complexity for this special case (for the requirement in Theorem \ref{thm_sample_cmpl}) is $n=O\left( (C_{max}\sqrt m+1)\frac{1}{\epsilon^2} \log \frac {1}\delta+ \sqrt{C_{max}}\frac{\sqrt{m\log (1/\delta)}+\log(1/\delta)}{\epsilon^{1.5}} \right)$, and the true sample complexity, as described in Corollary \ref{cor_main}, is obtained by replacing $\delta$ with $\frac {\delta}{m}$.
